How benign is benign overfitting?

We investigate two causes for adversarial vulnerability in deep neural networks: bad data and (poorly) trained models. When trained with SGD, deep neural networks essentially achieve zero training error, even in the presence of label noise, while also exhibiting good generalization on natural test data, something referred to as benign overfitting [2, 10]. However, these models are vulnerable to adversarial attacks. We identify label noise as one of the causes for adversarial vulnerability, and provide theoretical and empirical evidence in support of this. Surprisingly, we find several instances of label noise in datasets such as MNIST and CIFAR, and that robustly trained models incur training error on some of these, i.e. they don't fit the noise. However, removing noisy labels alone does not suffice to achieve adversarial robustness. Standard training procedures bias neural networks towards learning "simple" classification boundaries, which may be less robust than more complex ones. We observe that adversarial training does produce more complex decision boundaries. We conjecture that in part the need for complex decision boundaries arises from sub-optimal representation learning. By means of simple toy examples, we show theoretically how the choice of representation can drastically affect adversarial robustness.

==> adv_train.tex <==
\section{Investigating Adversarially Trained Models}
\label{sec:invest-advers-train}

One of the most commonly used techniques to increase adversarial
robustness of deep neural networks is Adversarial
Training~\citep{madry2018towards}~(\AT). However, \AT is
known to provide robustness at a cost to clean
accuracy~\citep{Raghunathan2019,tsipras2018robustness}. In~\cref{tab:accs-robust-models},  
we show that both the clean train and test accuracies drop with increasing strength of the PGD adversary
used for Adversarial Training~(\AT) a ResNet50 model on CIFAR-10. 
With the insights from the previous section, here we investigate
whether \AT  utilizes the phenomenon described in the previous section
to gain robustness.

\begin{figure}[t]
  \centering
 \begin{subfigure}[b]{0.53\linewidth}
 \begin{subfigure}[t]{0.99\linewidth}
    \includegraphics[width=0.24\linewidth]{./figures/adv_mis_tr_te/ostrich.png}
    \includegraphics[width=0.24\linewidth]{./figures/adv_mis_tr_te/water_birds.png}
    \includegraphics[width=0.24\linewidth]{./figures/adv_mis_tr_te/wheat_bird.png}
    \includegraphics[width=0.24\linewidth]{./figures/adv_mis_tr_te/cat_eye.png}
  \end{subfigure}
  \begin{subfigure}[t]{0.99\linewidth}
    \includegraphics[width=0.24\linewidth]{./figures/adv_mis_tr_te/b54.png}
    \includegraphics[width=0.24\linewidth]{./figures/adv_mis_tr_te/wheel_truck.png}
    \includegraphics[width=0.24\linewidth]{./figures/adv_mis_tr_te/red_truck.png}
    \includegraphics[width=0.24\linewidth]{./figures/adv_mis_tr_te/eye_deer.png}
  \end{subfigure}
  \begin{subfigure}[t]{0.99\linewidth}
    \includegraphics[width=0.24\linewidth]{./figures/adv_mis_tr_te/yellow_cat.png}
    \includegraphics[width=0.24\linewidth]{./figures/adv_mis_tr_te/boeing.png}
    \includegraphics[width=0.24\linewidth]{./figures/adv_mis_tr_te/green_wall_cat.png}
\includegraphics[width=0.24\linewidth]{./figures/adv_mis_tr_te/water_deer.png}
\end{subfigure}
\caption*{CIFAR10}
\end{subfigure}
\begin{subfigure}[b]{0.45\linewidth}
  \centering \def\svgwidth{0.99\linewidth}
  \input{./figures/adv_mis_tr_te_mnist.pdf_tex}
  \caption*{MNIST}
\end{subfigure}
\caption{Each pair is a  training~(left)
    and  test~(right) image mis-classified by the adversarially
    trained model. They were both correctly classified
    by the naturally-trained model.}
\end{figure}










\paragraph{Adversarial Training avoids memorizing rare examples}

Our hypothesis is that one of the effects of adversarial training is
to not \emph{memorize} rare examples, which would otherwise be
memorized by a naturally trained model. We use the same definition for
memorization of ~\emph{rare} samples as in~\citet{Feldman2019} but the
underlying intuition is that certain examples in the training set
belong to rare sub-populations~(eg. a special kind of cat) and this sub-population is
sufficiently distinct from the rest of the examples of that class in
the training dataset~(other cats in the dataset). This can quantified
by a quantity called~\emph{self-influence}. However, examples
from that sub-population are also present in the test-set and
\emph{memorizing} those rare training examples reduces the test error on those
examples. \AT, by not memorizing these rare samples,
only learns the major dominant features of each class~\citep{Santurkar2019} and this
helps in robustness.  However, as described above, this results in
mis-classifications of those rare sub-populations in the test set
leading to increasing test error.

To validate this hypothesis, we show a) Adversarially trained ResNet50
o CIFAR10, doesn't memorize certain rare training samples, and as a
result mis-classifies similar test-set samples. b) Adversarially
Trained CNN model on MNIST mis-classifies the naturally existing
label-noise samples in MNIST as well as certain odd-looking digits. c)
The self-influence of the  In~\cref{fig:cifar_self_influence}, we first show that the
self-influence of training samples, which indicates the need to memorization
those samples, is higher for data points that are mis-classified on
the train dataset by the adversarially trained model as compared to
the distribution of self-influence on the entire train dataset. This
supports our hypothesis that adversarial training excludes fitting
these rare~(or need to be memorized) samples.
\begin{figure}[t]
  \centering
  \begin{subfigure}[t]{0.24\linewidth}
        \centering \def\svgwidth{0.99\linewidth}
        \input{./figures/self_influence_car.pdf_tex}
        \caption*{CAR}
      \end{subfigure}
      \begin{subfigure}[t]{0.24\linewidth}
        \centering \def\svgwidth{0.99\linewidth}
        \input{./figures/self_influence_horse.pdf_tex}
        \caption*{HORSE}
      \end{subfigure}
      \begin{subfigure}[t]{0.24\linewidth}
        \centering \def\svgwidth{0.99\linewidth}
        \input{./figures/self_influence_ship.pdf_tex}
        \caption*{SHIP}
      \end{subfigure}
      \begin{subfigure}[t]{0.24\linewidth}
        \centering \def\svgwidth{0.99\linewidth}
        \input{./figures/self_influence_truck.pdf_tex}
        \caption*{TRUCK}
      \end{subfigure}
    \caption{Fraction of train points that have a self-influence
      greater than $s$ is plotted versus $s$. The blue line represents
      the points mis-classified by a adversarially trained model. The
      orange lines shows the distribution of self-influence for all
      points in the dataset~(of the concerned class).  }
    \label{fig:cifar_self_influence}\end{figure}


Next, we show that though ignoring these rare samples helps in
adversarial robustness, it hurts the test
accuracy. In~\cref{fig:adv-train-test-mis-class}, we  show some
examples from 6 classes of images from CIFAR10 dataset. Each pair of image contains a
mis-classified test image and the  mis-classified training image
responsible for it. The model used here is a AT model with
$\ell_2$-adversary with an $\epsilon=0.25$. We find these images by
searching for each training image, the test image that would have the
highest increase in loss when that training image would be omitted
from training. We were grateful to get this data from~\citet{Feldman2019}.

\begin{remark}
  We can also observe this in an experiment on MNIST where we randomly
  assigned labels to 15\% of the dataset. A naturally trained models
  achieved $100\%$ accuracy on this dataset whereas an adversarially
  trained model  mis-classified $997$ examples in the training set
  after the same training regime. Out of these $997$ samples, $994$
  belonged to the set of examples whose labels were randomized.
\end{remark}

This behaviour is also observed more clearly in a simple
distribution. In~\cref{fig:simple_adv_train}, we create a binary
classification problem where there are some \emph{rare}
sub-populations~(smaller circles) and some more dominant~(bigger
circles) sub-populations and train a wide shallow NN and a deep NN
with adversarial training and natural training. The decision
boundaries show that adversarial training creates decision regions
with larger margins but in the process ignores some of the rare
regions whereas natural training classifies almost each region
accurately but creates a decision regions with smaller margins. We
explore this topic in the next section.

\begin{figure}[t]
  \begin{subfigure}[t]{0.495\linewidth}
    \begin{subfigure}[t]{0.495\linewidth}
      \centering \def\svgwidth{0.999\linewidth}
      \input{./figures/adv_shallow_wide_nn_decision_region.pdf_tex}
      \caption*{AT}
    \end{subfigure}
    \begin{subfigure}[t]{0.495\linewidth}
      \centering \def\svgwidth{0.999\linewidth}
      \input{./figures/nat_shallow_wide_nn_decision_region.pdf_tex}
      \caption*{NAT}
    \end{subfigure}\caption{Shallow Wide NN}
  \end{subfigure}
  \begin{subfigure}[t]{0.495\linewidth}
    \begin{subfigure}[t]{0.495\linewidth}
      \centering \def\svgwidth{0.999\linewidth}
      \input{./figures/adv_deep_nn_decision_region.pdf_tex}
      \caption*{AT}
    \end{subfigure}
    \begin{subfigure}[t]{0.495\linewidth}
      \centering \def\svgwidth{0.999\linewidth}
      \input{./figures/nat_deep_nn_decision_region.pdf_tex}
      \caption*{NAT}
    \end{subfigure}\caption{Deep NN}
  \end{subfigure}
  \label{fig:simple_adv_train}
  \caption{Adversarial training~(AT) leads to larger margin, and thus
    adversarial robustness around high density regions~(larger
    circles) but causes training error on low
    density sub-populations~(smaller circles) whereas naturally
    trained models~(NAT) minimizes the training error but leads to
    regions with very small margins.}
\end{figure}




==> hardness.tex <==
\section{Hardness of Improper Robust Learning}
\label{sec:hardn-impr-robust}

We define the  concept class $\cC$ of concepts
$c_S:\bs{0,N}\rightarrow
\bc{0,1}$ such that
\begin{equation}
  \label{eq:parity_concept}
  c_S\br{\vec{x}}=\begin{cases}
    0,
    &\text{if}\br{\langle\bs{\vec{x}}\rangle_b~\mathrm{XOR}~S}~\text{
      is odd.}\\
    0 &~\text{o.w.}
    \end{cases}
\end{equation}
where $\bs{\cdot}:\bs{0,N}\rightarrow\bc{0,\cdots,N}$ rounds a decimal
to its nearest
integer,$\langle\cdot\rangle_b:\bc{0,\cdots,N}\rightarrow\bc{0,1}^n$
returns the binary encoding of the integer,  $N=2^n,~S\in\bc{0,1}^n$
and $n\in\bZ_+$. It is essentially the class of parity functions defined on the nearest
integer. We look at a binary classification problem where  data
distribution $\cD_{S,\zeta}\subseteq\bc{\cX,\cY}$, for
$\zeta\subseteq\bs{0,\cdots}$ is such that the support of $\cX_\zeta$ is a union of
intervals. 
\begin{equation}
  \label{eq:dist_union_int}
  \supp{\cX}_\zeta=\bigcup_{j\in\zeta}I_j\text{ where }
  I_j\subseteq\br{j-\frac{1}{4}, j+\frac{1}{4}}
\end{equation}
and each sample from $\br{\vec{x},y}~\sim\cD_{S,\zeta}$ is created by sampling
$\vec{x}$ uniformly $\cX$ and assigning $y=c_S\br{\vec{x}}$. Finally, we create
$\cD_{S,\zeta}^\eta$ -a noisy version of $\cD_{S,\zeta}$, by flipping $y$ in each sample
$\br{x,y}$ with probability $\eta<\frac{1}{2}$.

The
objective of the learning problem is to, given oracle access to
$\cD_{S,\zeta}^\eta$, output a function $f:\bs{0,\cdots,N}\rightarrow\bc{0,1}$
efficiently, such that $f$ has low test error and is adversarially
robust on $\cD_{S,\zeta}$. We define adversarial
error~$\radv{\delta}{f;\cD_{S,\zeta}} = \bP_{\br{x,y}\sim D_S}\bs{\exists
  z~\text{s.t.}\abs{z-x}\le\delta\wedge f\br{x}\neq f\br{z}}$.


Before proceeding further, we define the concept class of union of
$k$ intervals on the real line as $\cU^k$. Each concept in $\cU^k$
can be written as a set of $k$ disjoint intervals where each
interval is associated with a label -
$\bc{\br{I_1,y_1},\cdots,\br{I_k,y_k}}$ such that the intervals are
pairwise-disjoint and their union covers the entire real line-segment
$\bs{0,N}$. The algorithm predicts on a new
point by returning the label of the interval the point falls
in. Given a binary classification problem, $\cU^k$~(for an
appropriate $k$) is a natural target concept class to learning from.


  
\begin{restatable}{lem}{exactrobust}
  Any $f$ that learns this
  distribution~\emph{exactly}  is adversarially robust for all
  $\delta< \frac{1}{4}$. \todo{Do this for $\epsilon$ error.}
\end{restatable}
First, we look at the simpler noise-less case i.e. for the
distribution $\cD_{S,\zeta}^0$~($\abs{\zeta}=N$). We show that there exists a PAC algorithm
that can learn a target concept$f\in\cC$~\cref{eq:parity_concept} in
time $\poly{\log{N}}$ such that $f$ has small test error and is
adversarially robust. However, is we view this as a union of $N$
intervals learning problems, it would require $\poly{N}$ samples.


\begin{lem}\label{eq:no_noise_robustness}
  Given a Distribution $\cD_{S,\zeta}^0$, where $\abs{\zeta}=N$ there exists a PAC learning
  algorithm that outputs a hypothesis $f$ such that
  $\risk{\cD_{S,\eta}}{f}\le\epsilon,~\radv{\gamma}{f;\cD_{S,\eta}}=0$
  for all $\gamma<\frac{1}{4}$  in time $\poly{\log{N}}$ whereas a union of intervals learning
  algorithm would need time $\Om{\poly{N}}$ to return a concept
  $h\in\cU^N$ with $\risk{\cD_{S,\zeta}}{h}\le\epsilon$.~{\color{red} I
    think such a concept would also not be necessarily robust but will
  have to think about how to prove it See example 2 in~\url{https://arxiv.org/pdf/2003.06121.pdf}}
\end{lem}
\begin{proof}
  {\color{red} TODO}
\end{proof}
~\cref{eq:no_noise_robustness} shows that without intrinsic knowledge
of the true target concept, while it might be still possible to obtain
a PAC-learning algorithm  the sample complexity can be exponentially
large as compared to another PAC-learning algorithm that has hidden
knowledge regarding the structure of the problem. In addition, such
biases can also make the concept more adversarially robust. In some sense, a
similar parallelism can be drawn between the ability of humans to use
very few samples to learn concepts whereas current machine learning
systems requires orders of magnitudes more observations to reach a
comparable level of performance.  Perhaps this is because, the human
cognitive learning system uses other intrinsic biases in its visual
recognition system, which not only allows it to learn concepts with
fewer examples but also encodes what we commonly refer
to~\emph{perceptual distance} and makes it robust to adversarial examples.



\paragraph{Noisy Label Setting}

Next, we look at the noisy label setting. We show in~\cref{lem:noisy_parity}, that when
armed with the intrinsic knowledge regarding the construction of $\cD$,
there exists an algorithm that outputs a
hypothesis in $\cC$ which has both $0$ risk and $0$ adversarial risk
with high probability on the support of the observed distribution
~($\zeta$) but not $0$ training error.

The same algorithm when run on a distribution whose support $\zeta$
has atleast $\softO{\frac{n}{\epsilon}}$ runs in polynomial time to
return a hypothesis in $\cC$ which incurs an error less than
$\epsilon$ and $0$ adversarial error.

However, when learning a union of intervals hypothesis~($\cU$), we
show in~\cref{lem:noisy_interval} that there is a hypothesis in $\cU$ that has $0$ training error,
and less than $\epsilon$ test error but incurs an adversarial risk
greater than $\gamma - \epsilon$ when attacked with an adversary,
whose perturbation budget is bounded by $\gamma<\frac{1}{4}$. In fact,
for any classifier in $\cH$, that achieves zero traiing error, we show
that the adversarial risk is lower bounded by $\gamma-\epsilon$ where
$\epsilon$ is the test error.



\begin{restatable}{lem}{noisyparity}\label{lem:noisy_parity}
  There exists a  learning algorithm $\cA$ such that given
  access to $\cD_{S,\zeta}^\eta$ through an example oracle
  $\mathrm{EX}\br{\cD_{S,\zeta}^\eta}$ returns a hypothesis $f\in\cC$
  in time
  $\bigO{\abs{\zeta}\br{\frac{1}{\frac{1}{2}-\eta}}^2
    \log{\frac{\abs{\zeta}}{\delta}}}$ such that with probability
  $1-\frac{2\delta}{3}$, we have that $\risk{\cD_{S,\zeta}}{f}=0$ and
  $\radv{\gamma}{f;\cD_{S,\zeta}}=0$ for all $\gamma<\frac{1}{4}$.

  
  Further if $\abs{\zeta}=\bigO{\frac{1}{\epsilon}  \log\frac{3}{\delta}+
      \frac{n}{\epsilon}\log\frac{1}{\epsilon}}$ then given access to
  $\mathrm{EX}\br{\cD_{S,\zeta}^\eta}$, 
  $\cA$ runs in time
  $\bigO{\poly{n\log{n},\frac{1}{\epsilon}\log{\frac{1}{\epsilon}},
      \frac{1}{\delta}\log{\frac{1}{\delta}},\br{\frac{1}{\frac{1}{2}-\eta}}^2}}$ 
  to return $f$ such that 
  $\risk{f}{\cD_{S,\tilde{\zeta}}}\le\epsilon$ and
  $\radv{\cD_{S,\zeta}}{f}=0$ with probability at-least
  $1-\delta$ for any $\tilde{z}\subseteq{0,\cdots, 2^n}$.
\end{restatable}



\begin{restatable}{lem}{noisyinterval}\label{lem:noisy_interval}
Given a set of $m$ examples denoted as $\cS_m$ obtained through an example oracle
 $\mathrm{EX}\br{\cD_{S,\zeta}^\eta}$ for $\eta<\frac{1}{16}$ where
 $m\ge\frac{1}{2\epsilon^2\br{1-16\eta}}\br{\abs{\zeta}+\log{\frac{1}{\delta}}}$,
 with probability $1-\delta-e^{-75}$, where the
probability is over the randomization in $\mathrm{EX}$,  there exists a concept
 $h\in\cU=\bigcup_{i=1}^\infty\cU^{i}$ such that a) $h$  is consistent on 
 $\cS_m$ , b) has $\risk{\cD_{S,\zeta}}{h}\le\epsilon$, and
 has c) $\radv{\gamma}{h;\cD_{S,\zeta}}\ge\gamma-\epsilon$.
 
 Further \emph{any}  hypothesis $h\in  \cU$ that is consistent with $\cS_m$ and has risk less
 than $\epsilon$ has adversarial risk 
 $\radv{\gamma}{h;\cS_{S,\zeta}}\ge\gamma - \epsilon$ for
 $\gamma<\frac{1}{4}$.

 {\color{red} (Possible?) For any $\zeta,
   \abs{\zeta}=\bigO{\poly{n}}$, there exists a $S$ such that, for any
   $m$ examples obtained through calls to
   $\mathrm{EX}\br{\cD_{S,\zeta}^\eta}$ -
   denoted as $\cS_m$, for all
   $h\in\cU$ that is consistent on $\cS_m$,
   $\risk{\cD_{S,\bs{0,\cdots,N}}}{h}>\bigO{\frac{1}{\abs{\zeta}}}$ }
\end{restatable}




==> notation.tex <==

\section{Notations and Related Works}
\label{sec:notations}

Throughout the paper, we use $\cD$ to denote a distribution
over~$\cX\times\bc{0,1}$, where $\cX$ is the input space. $\cC$ and
$\cH$ represents concept classes from $\cX$ to $\bc{0,1}$. We use $n$
to represent the dimension of the problem, and $m$ to denote the size
of the training set,  which is denoted by $\cS_m$. We represent the test error on a distribution $\cD$
of a classifier $f$ as $\risk{\cD}{f}$. The perturbation radius is
usually denoted by $\gamma$ and the adversarial risk of a
classifier $f$ on a distribution $\cD$ for a adversarial perturbation
radius of $\gamma$ is $\radv{\gamma}{f;\cD}$

Some other commonly used notations include $\eta$ to represent the level of label noise,
$\epsilon$ to represent the test error, and $\delta$ to represent the
represent the probability of failure. These are standard notations in
the~\emph{Probably Approximately Correct}~(PAC) learning
literature. In the presence of $\eta$-noisy labels, the training set
is represented by $\cS_m^\eta$





\textbf{Other Related Work}: In this section, we discuss some other
        works that are related to this paper. While, we discussed the
        most related works in the main paper, due to lack of space we
        discuss the rest here. ~\citep{montasser19a} established that there
	are concept classes with finite VC dimensions i.e. are \emph{properly}
	PAC-learnable but are only \emph{improperly} robustly PAC learnable. This
	implies that to learn the problem with small adversarial error, a different
	class of models~(or representations) needs to be used whereas for small
	natural test risk, the original model class~(or representation) can be used.
	Recent empirical works have also shown evidence towards
	this~(eg.~\citep{Sanyal2020LR}).


        \citet{pmlr-v97-hanin19a} have shown that
	though the number of possible linear regions that can be created by a deep
	ReLU network is exponential in depth, in practice for networks trained with
	SGD this tends to grow only linearly thus creating much simpler decision
        boundaries than is possible  due to sheer expresssivity of
        deep networks. Experiments on the data models from our
	theoretical settings indeed show that adversarial training indeed produces more
	``complex'' decision boundaries

        \citesec{jacobsen2018excessive} have discussed that excesssive
        invariance in neural networks might increase adversarial
        error. However, their argument is that excessive invariance
        can allow sufficient changes in the semantically important
        features without changing the network's prediction. They
        describe this as Invariance-based adversarial examples as
        opposed to perturbation based adversarial examples. We show
        that excessive ~(incorrect) invariance might also result in
        perturbation based adversarial examples.

        Another contemporary
        work~\citesec{Geirhos2020} discusses a phenomenon they refer to as~\emph{Shortcut
          Learning} where deep learning models perform very well on
        standard tasks like reducing classification error but fail to
        perform in more difficult real world situations. We discuss
        this in the context of models that have small test
        error but large adversarial error and provide and theoretical
        and empirical to discuss why one of the reasons for this is
        sub-optimal representation learning.



